The LAMOST Spectroscopic Survey of Supergiants in M31 and M33

We present systematic identifications of supergiants of M31/M33 based on massive LAMOST spectroscopic survey. Radial velocities of nearly 5000 photometrically selected M31/M33 supergiant candidates have been properly derived from the qualified spectra released in LAMOST DR10. By comparing their radial velocities with those predicted from the rotation curves of M31, as well as utilizing {\it Gaia} astrometric measurements to exclude foreground contaminations, 199 supergiant members in M31, including 168 `Rank1' and 31 `Rank2', have been successfully identified. This sample contains 62 blue supergiants (BSGs, all `Rank1'), 134 yellow supergiants (YSGs, 103 `Rank1' and 31 `Rank2') and 3 red supergiants (RSGs, all `Rank1'). For M33, we identify 84 supergiant members (56 `Rank1' and 28 `Rank2'), which includes 28 BSGs (all `Rank1'), 53 YSGs (25 `Rank1' and 28 `Rank2') and 3 RSGs (all `Rank1'). So far, this is one of the largest supergiant sample of M31/M33 with full optical wavelength coverage (3700 \textless $\lambda$ \textless 9100 \AA). This sample is valuable for understanding the star formation and stellar evolution under different environments.

==> readme <==
Dear Colleagues: 

The final publication layout will be produced by using raa.cls. 
Therefore, we strongly encourage you to prepare your LaTeX manuscript 
with this class file. Please unpack raa-package.tar.gz, it includes 

raa.cls        ---- RAA macro class file for LaTeX2e 
sample.tex     ---- a sample file using raa.cls (LaTeX source) 
sample.ps      ---- the PS file created by sample.tex in referee format  
sample.pdf     ---- the PDF file created by sample.tex in referee format  
readme         ---- this file  
f?.eps         ---- three demo figures used in the LaTeX template source
sample2.tex    ---- a sample file for using raa.bst
sample2_fig?.eps -- two demo figures used in sample2.tex
sample2.pdf    ---- the PDF file created by sample.tex in referee format
sample2.bbl    ---- bibliography file using by sample2.tex
bibtex.bib     ---- an example for bibtex file

natbib.sty     ---- This package reimplements the LaTeX \cite command
natnotes.pdf   ---- Brief reference sheet for Natbib (pdf)
raa.bst        ---- Bibliography style file 

Hope you enjoy the use of this macro. Your suggestions and comments are 
highly welcome. Thanks.

Editorial Office
E-mail:  raa@raa-journal.org

